IDA-UIE: An Iterative Framework for Deep Network-based Degradation Aware Underwater Image Enhancement

Underwater image quality is affected by fluorescence, low illumination, absorption, and scattering. Recent works in underwater image enhancement have proposed different deep network architectures to handle these problems. Most of these works have proposed a single network to handle all the challenges. We believe that deep networks trained for specific conditions deliver better performance than a single network learned from all degradation cases. Accordingly, the first contribution of this work lies in the proposal of an iterative framework where a single dominant degradation condition is identified and resolved. This proposal considers the following eight degradation conditions -- low illumination, low contrast, haziness, blurred image, presence of noise and color imbalance in three different channels. A deep network is designed to identify the dominant degradation condition. Accordingly, an appropriate deep network is selected for degradation condition-specific enhancement. The second contribution of this work is the construction of degradation condition specific datasets from good quality images of two standard datasets (UIEB and EUVP). This dataset is used to learn the condition specific enhancement networks. The proposed approach is found to outperform nine baseline methods on UIEB and EUVP datasets.

==> references.tex <==
\bibitem{sahu2014survey}
Pooja Sahu, Neelesh Gupta, and Neetu Sharma.
\newblock A survey on underwater image enhancement techniques.
\newblock {\em International Journal of Computer Applications}, 87(13), 2014.

\bibitem[Raveendran et al.(2021)]{raveendran2021underwater}
S. Raveendran, M. D. Patil, and G. K. Birajdar, "Underwater image enhancement: a comprehensive review, recent trends, challenges and applications," \textit{Artificial Intelligence Review}, vol. 54, pp. 5413-5467, 2021.

\bibitem{r9}
Oscar C.~Au, Lin Sun, Ruobing Zou, Wei Dai, and Sijin Li.
\newblock An improved method for color images enhancement considering HVS.
\newblock In {\em 2012 International Conference on Audio, Language and Image Processing}, pages 117--122. IEEE, 2012.

\bibitem{hasibuan2021contrast}
Z.~A.~Hasibuan, P.~N.~Andono, D.~Pujiono, R.~I.~M.~Setiadi, et al.
\newblock Contrast limited adaptive histogram equalization for underwater image matching optimization use SURF.
\newblock In {\em Journal of Physics: Conference Series}, volume 1803, number 1, page 012008. IOP Publishing, 2021.

\bibitem{a3}
Achmad Basuki and Nana Ramadijanti.
\newblock Improving auto level method for enhancement of underwater images.
\newblock In {\em 2016 International Conference on Knowledge Creation and Intelligent Computing (KCIC)}, pages 120--125. IEEE, 2016.

\bibitem[Fabbri et al.(2018)]{fabbri2018enhancing}
Fabbri, Cameron, Islam, Md Jahidul, and Sattar, Junaed.
\newblock {Enhancing underwater imagery using generative adversarial networks}.
\newblock In {\em 2018 IEEE International Conference on Robotics and Automation (ICRA)}, pages 7159-7165. IEEE, 2018.

\bibitem[Yang and Sowmya(2015)]{yang2015underwater}
Yang, Miao, and Sowmya, Arcot.
\newblock {An underwater color image quality evaluation metric}.
\newblock {\em IEEE Transactions on Image Processing}, 24(12):6062-6071, 2015.

\bibitem[Wang et al.(2015)]{wang2015patch}
Wang, Shiqi, Ma, Kede, Yeganeh, Hojatollah, Wang, Zhou, and Lin, Weisi.
\newblock {A patch-structure representation method for quality assessment of contrast changed images}.
\newblock {\em IEEE Signal Processing Letters}, 22(12):2387-2390, 2015.

\bibitem[Panetta et al.(2015)]{panetta2015human}
Panetta, Karen, Gao, Chen, and Agaian, Sos.
\newblock {Human-visual-system-inspired underwater image quality measures}.
\newblock {\em IEEE Journal of Oceanic Engineering}, 41(3):541-551, 2015.

\bibitem[Mittal et al.(2012)]{mittal2012making}
Mittal, Anish, Soundararajan, Rajiv, and Bovik, Alan C.
\newblock {Making a "completely blind" image quality analyzer}.
\newblock {\em IEEE Signal Processing Letters}, 20(3):209-212, 2012.

\bibitem[Sharma et al.(2023)]{sharma2023wavelength}
Sharma, Prasen, Bisht, Ira, and Sur, Arijit.
\newblock {Wavelength-based attributed deep neural network for underwater image restoration}.
\newblock {\em ACM Transactions on Multimedia Computing, Communications and Applications}, 19(1):1-23, 2023.

\bibitem[Islam et al.(2020)]{islam2020simultaneous}
Islam, Md Jahidul, Luo, Peigen, and Sattar, Junaed.
\newblock {Simultaneous enhancement and super-resolution of underwater imagery for improved visual perception}.
\newblock {\em arXiv preprint arXiv:2002.01155}, 2020.

% \bibitem[Badran and Torki(2023)]{10222895}
% Badran, Mohamed, and Torki, Marwan.
% \newblock {DAUT: Underwater Image Enhancement Using Depth Aware U-shape Transformer}.
% \newblock In {\em 2023 IEEE International Conference on Image Processing (ICIP)}, pages 1830-1834, 2023.

% \bibitem[Yan et al.(2023)]{10251985}
% H. Yan, Z. Zhang, J. Xu, T. Wang, P. An, A. Wang, and Y. Duan, "UW-CycleGAN: Model-Driven CycleGAN for Underwater Image Restoration," \textit{IEEE Transactions on Geoscience and Remote Sensing}, vol. 61, pp. 1-17, 2023.

\bibitem[Islam et al.(2020)]{9001231}
M. J. Islam, Y. Xia, and J. Sattar, "Fast Underwater Image Enhancement for Improved Visual Perception," \textit{IEEE Robotics and Automation Letters}, vol. 5, no. 2, pp. 3227-3234, 2020.

\bibitem[Li et al.(2019)]{li2019underwater}
C. Li, C. Guo, W. Ren, R. Cong, J. Hou, S. Kwong, and D. Tao, "An underwater image enhancement benchmark dataset and beyond," \textit{IEEE Transactions on Image Processing}, vol. 29, pp. 4376-4389, 2019.

\bibitem[Yi et al.(2024)]{yi2024no}
X. Yi, Q. Jiang, and W. Zhou, "No-reference quality assessment of underwater image enhancement," \textit{Displays}, vol. 81, pp. 102586, 2024.

\bibitem[Li et al.(2024)]{li2024underwater}
Y. Li, D. Li, Z. Gao, S. Wang, Q. Jiao, and others, "Underwater image enhancement utilizing adaptive color correction and model conversion for dehazing," \textit{Optics \& Laser Technology}, vol. 169, pp. 110039, 2024.

\bibitem[Hu et al.(2024)]{hu2024texture}
S. Hu, Z. Cheng, G. Fan, M. Gan, and C. L. P. Chen, "Texture-aware and color-consistent learning for underwater image enhancement," \textit{Journal of Visual Communication and Image Representation}, vol. 98, pp. 104051, 2024.

\bibitem[Xiao et al.(2024)]{xiao2024underwater}
S. Xiao, X. Shen, Z. Zhang, J. Wen, M. Xi, and J. Yang, "Underwater image classification based on image enhancement and information quality evaluation," \textit{Displays}, vol. 82, pp. 102635, 2024.

\bibitem[Zheng et al.(2024)]{zheng2024illumination}
R. Zheng, J. Miao, H. Zhang, X. Liu, and D. Tan, "An illumination adaptive underwater image enhancement method," in \textit{International Conference on Algorithm, Imaging Processing, and Machine Vision (AIPMV 2023)}, vol. 12969, pp. 442-449, 2024.

\bibitem[Mao et al.(2016)]{mao2016image}
X. Mao, C. Shen, and Y.-B. Yang, "Image restoration using very deep convolutional encoder-decoder networks with symmetric skip connections," \textit{Advances in Neural Information Processing Systems}, vol. 29, 2016.

\bibitem[Sun et al.(2019)]{sun2019deep}
X. Sun, L. Liu, Q. Li, J. Dong, E. Lima, and R. Yin, "Deep pixel-to-pixel network for underwater image enhancement and restoration," \textit{IET Image Processing}, vol. 13, no. 3, pp. 469-474, 2019.

\bibitem[Kumar(2020)]{kumarunderwater}
V. S. Kumar, "An Underwater Image Dehazing Method using Dark Channel Prior," \textit{Journal}, vol. XX, pp. XX-XX, 2020.

% \bibitem[Liu et al.(2019)]{liu2019real}
% R. Liu, X. Fan, M. Zhu, M. Hou, and Z. Luo, "Real-world underwater enhancement: challenges, benchmarks, and solutions," \textit{arXiv preprint arXiv:1901.05320}, 2019.



\bibitem{6247661}
Cosmin Ancuti, Codruta Orniana Ancuti, Tom Haber, and Philippe Bekaert.
\newblock Enhancing underwater images and videos by fusion.
\newblock In {\em 2012 IEEE Conference on Computer Vision and Pattern Recognition}, pages 81--88. IEEE, 2012.

\bibitem{8917818}
Chongyi Li, Chunle Guo, Wenqi Ren, Runmin Cong, Junhui Hou, Sam Kwong, and Dacheng Tao.
\newblock An Underwater Image Enhancement Benchmark Dataset and Beyond.
\newblock {\em IEEE Transactions on Image Processing}, 29:4376--4389, 2020.
\bibitem{islam2020fast}

Md Jahidul Islam, Youya Xia, and Junaed Sattar.
\newblock Fast underwater image enhancement for improved visual perception.
\newblock {\em IEEE Robotics and Automation Letters}, 5(2):3227--3234, 2020.

\bibitem[Yang et al.(2020)]{yang2020underwater}
M. Yang, K. Hu, Y. Du, Z. Wei, Z. Sheng, and J. Hu, "Underwater image enhancement based on conditional generative adversarial network," \textit{Signal Processing: Image Communication}, vol. 81, pp. 115723, 2020.

\bibitem[Hu et al.(2022)]{hu2022overview}
K. Hu, C. Weng, Y. Zhang, J. Jin, and Q. Xia, "An overview of underwater vision enhancement: from traditional methods to recent deep learning," \textit{Journal of Marine Science and Engineering}, vol. 10, no. 2, pp. 241, 2022.

% \bibitem[Abin et al.(2021)]{abin2021fusion}
% D. Abin, B. Gulabani, C. Joshi, S. Damle, and S. Gengaje, "Fusion based approach for Underwater Image Enhancement," in \textit{2021 International Conference on Communication information and Computing Technology (ICCICT)}, pp. 1-5, 2021.

\bibitem[Wang et al.(2020)]{wang2020underwater}
Z. Wang, X. Xue, L. Ma, and X. Fan, "Underwater image enhancement based on dual U-net," in \textit{2020 8th International Conference on Digital Home (ICDH)}, pp. 141-146, 2020.

% \bibitem[Wang et al.(2017)]{wang2017deep}
% Y. Wang, J. Zhang, Y. Cao, and Z. Wang, "A deep CNN method for underwater image enhancement," in \textit{2017 IEEE international conference on image processing (ICIP)}, pp. 1382-1386, 2017.

\bibitem{yussof2013performing}
W.~N.~J.~H.~W.~Yussof, M.~S.~Hitam, E.~A.~Awalludin, and Z.~Bachok.
\newblock Performing contrast limited adaptive histogram equalization technique on combined color models for underwater image enhancement.
\newblock {\em International Journal of Interactive Digital Media}, 1(1):1--6, 2013.

\bibitem{hassan2021retinex}
Najmul Hassan, Sami Ullah, Naeem Bhatti, Hasan Mahmood, and Muhammad Zia.
\newblock The Retinex based improved underwater image enhancement.
\newblock {\em Multimedia Tools and Applications}, 80:1839--1857, 2021.



\bibitem{deperlioglu2018underwater}
Omer Deperlioglu, Utku Kose, and G.~Emre Guraksin.
\newblock Underwater image enhancement with HSV and histogram equalization.
\newblock {\em Image}, 1(4):461--465, 2018.

% \bibitem{wang2019experimental}
% Yan Wang, Wei Song, Giancarlo Fortino, Li-Zhe Qi, Wenqiang Zhang, and Antonio Liotta.
% \newblock An experimental-based review of image enhancement and image restoration methods for underwater imaging.
% \newblock {\em IEEE Access}, 7:140233--140251, 2019.

% \bibitem{schettini2010underwater}
% Raimondo Schettini and Silvia Corchs.
% \newblock Underwater image processing: state of the art of restoration and image enhancement methods.
% \newblock {\em EURASIP Journal on Advances in Signal Processing}, 2010:1--14, 2010.



% \bibitem{r2}
% Amal AbuNaser, Iyad Abu Doush, Nahed Mansour, and Sawsan Alshattnawi.
% \newblock Underwater image enhancement using particle swarm optimization.
% \newblock {\em Journal of Intelligent Systems}, 24(1):99--115, 2015.

% \bibitem{r3}
% Jonghyun Ahn, Shinsuke Yasukawa, Takashi Sonoda, Tamaki Ura, and Kazuo Ishii.
% \newblock Enhancement of deep-sea floor images obtained by an underwater vehicle and its evaluation by crab recognition.
% \newblock {\em Journal of Marine Science and Technology}, 22:758--770, 2017.

\bibitem{r4}
Raj S.~M.~Alex, S.~Deepa, and M.~H.~Supriya.
\newblock Underwater image enhancement using CLAHE in a reconfigurable platform.
\newblock In {\em OCEANS 2016 MTS/IEEE Monterey}, pages 1--5. IEEE, 2016.

\bibitem{r5}
Cosmin Ancuti, Codruta Orniana Ancuti, Tom Haber, and Philippe Bekaert.
\newblock Enhancing underwater images and videos by fusion.
\newblock In {\em 2012 IEEE Conference on Computer Vision and Pattern Recognition}, pages 81--88. IEEE, 2012.

% \bibitem{r6}
% Codruta O.~Ancuti, Cosmin Ancuti, Christophe De Vleeschouwer, and Philippe Bekaert.
% \newblock Color balance and fusion for underwater image enhancement.
% \newblock {\em IEEE Transactions on Image Processing}, 27(1):379--393, 2017.

% \bibitem{r7}
% Saeed Anwar and Chongyi Li.
% \newblock Diving deeper into underwater image enhancement: A survey.
% \newblock {\em Signal Processing: Image Communication}, 89:115978, 2020.

% \bibitem{r8}
% Jun Ao and Chunbo Ma.
% \newblock Adaptive stretching method for underwater image color correction.
% \newblock {\em International Journal of Pattern Recognition and Artificial Intelligence}, 32(02):1854001, 2018.



\bibitem{a1}
Kamil Zakwan Mohd Azmi, Ahmad Shahrizan Abdul Ghani, Zulkifli Md Yusof, and Zuwairie Ibrahim.
\newblock Natural-based underwater image color enhancement through fusion of swarm-intelligence algorithm.
\newblock {\em Applied Soft Computing}, 85:105810, 2019.

% \bibitem{a2}
% Wagner Barros, Erickson R.~Nascimento, Walysson V.~Barbosa, and Mario F.~M.~Campos.
% \newblock Single-shot underwater image restoration: A visual quality-aware method based on light propagation model.
% \newblock {\em Journal of Visual Communication and Image Representation}, 55:363--373, 2018.


% \bibitem{a4}
% Asi Elad and Ron Kimmel.
% \newblock On bending invariant signatures for surfaces.
% \newblock {\em IEEE Transactions on Pattern Analysis and Machine Intelligence}, 25(10):1285--1295, 2003.

\bibitem{a5}
Bastiaan J.~Boom, Phoenix X.~Huang, Cigdem Beyan, Concetto Spampinato, Simone Palazzo, Jiyin He, Emmanuelle Beauxis-Aussalet, Sun-In Lin, Hsiu-Mei Chou, Gayathri Nadarajan, et al.
\newblock Long-term underwater camera surveillance for monitoring and analysis of fish populations.
\newblock {\em VAIB12}, 2012.

% \bibitem{a6}
% Mohcine Boudhane and Benayad Nsiri.
% \newblock Underwater image processing method for fish localization and detection in submarine environment.
% \newblock {\em Journal of Visual Communication and Image Representation}, 39:226--238, 2016.

% \bibitem{a7}
% Aysun Ta{\c{s}}yap{\i} {\c{C}}elebi and Sarp Ert{\"u}rk.
% \newblock Visual enhancement of underwater images using Empirical Mode Decomposition and wavelet denoising.
% \newblock In {\em 2012 20th Signal Processing and Communications Applications Conference (SIU)}, pages 1--4. IEEE, 2012.

% \bibitem{a8}
% Cheng-Hao Chang, I-Chang Huang, Mu-Fan Lin, and Shiann-Rong Kuang.
% \newblock Design and implementation of a low-cost guided image filter for underwater image enhancement.
% \newblock In {\em 2017 IEEE Conference on Dependable and Secure Computing}, pages 296--299. IEEE, 2017.

% \bibitem{a9}
% Yuzhang Chen and Kecheng Yang.
% \newblock MAP-regularized robust reconstruction for underwater imaging detection.
% \newblock {\em Optik}, 124(20):4514--4518, 2013.

% \bibitem{b1}
% Yuzhang Chen, Min Xia, Wei Li, Xiaohui Zhang, and Kecheng Yang.
% \newblock Comparison of point spread models for underwater image restoration.
% \newblock {\em Optik}, 123(9):753--757, 2012.

% \bibitem{b2}
% Zhe Chen, Huibin Wang, Jie Shen, Xiaofang Li, and Lizhong Xu.
% \newblock Region-specialized underwater image restoration in inhomogeneous optical environments.
% \newblock {\em Optik}, 125(9):2090--2098, 2014.

% \bibitem{b3}
% John Y.~Chiang and Ying-Ching Chen.
% \newblock Underwater image enhancement by wavelength compensation and dehazing.
% \newblock {\em IEEE Transactions on Image Processing}, 21(4):1756--1769, 2011.

% \bibitem{b4}
% John Y.~Chiang, Ying-Ching Chen, and Yung-Fu Chen.
% \newblock Underwater image enhancement: using wavelength compensation and image dehazing (WCID).
% \newblock In {\em Advanced Concepts for Intelligent Vision Systems: 13th International Conference, ACIVS 2011, Ghent, Belgium, August 22-25, 2011. Proceedings 13}, pages 372--383. Springer, 2011.

% \bibitem{b5}
% Suxia Cui, Yu Zhou, Yonghui Wang, and Lujun Zhai.
% \newblock Fish detection using deep learning.
% \newblock {\em Applied Computational Intelligence and Soft Computing}, 2020:1--13, 2020.

% \bibitem{b6}
% Shaveta Dargan, Munish Kumar, Maruthi Rohit Ayyagari, and Gulshan Kumar.
% \newblock A survey of deep learning and its applications: a new paradigm to machine learning.
% \newblock {\em Archives of Computational Methods in Engineering}, 27:1071--1092, 2020.

% \bibitem{b7}
% Xiangyu Deng, Huigang Wang, Xing Liu, and Qingyue Gu.
% \newblock State of the art of the underwater image processing methods.
% \newblock In {\em 2017 IEEE International Conference on Signal Processing, Communications and Computing (ICSPCC)}, pages 1--6. IEEE, 2017.

% \bibitem{b8}
% Xueyan Ding, Yafei Wang, Zheng Liang, Jun Zhang, and Xianping Fu.
% \newblock Towards underwater image enhancement using super-resolution convolutional neural networks.
% \newblock In {\em Internet Multimedia Computing and Service: 9th International Conference, ICIMCS 2017, Qingdao, China, August 23-25, 2017, Revised Selected Papers}, pages 479--486. Springer, 2018.

% \bibitem{b9}
% Sonal Dixit, Sandeep Kumar Tiwari, and Pankaj Sharma.
% \newblock Underwater image enhancement using DCP with ACCLAHE and homomorphism filtering.
% \newblock In {\em 2016 International Conference on Signal Processing, Communication, Power and Embedded System (SCOPES)}, pages 2042--2046. IEEE, 2016.


% \bibitem{c1}
% Amanda Duarte, Felipe Codevilla, Joel De O.~Gaya, and Silvia S.~C.~Botelho.
% \newblock A dataset to evaluate underwater image restoration methods.
% \newblock In {\em OCEANS 2016-Shanghai}, pages 1--6. IEEE, 2016.

% \bibitem{c2}
% Nisheeth Dubey, Sandeep Kumar Tiwari, and Pankaj Sharma.
% \newblock A hybrid DCT-DHE approach for enhancement of low contrast underwater images.
% \newblock In {\em 2017 International Conference on Recent Innovations in Signal processing and Embedded Systems (RISE)}, pages 304--309. IEEE, 2017.

% \bibitem{c3}
% Pushkresh Kumar Dwivedi, Biswajit Paul, and Dibyendu Ghoshal.
% \newblock Notice of removal: underwater image enhancement using distance factor estimation.
% \newblock In {\em 2015 International Conference on Electrical, Electronics, Signals, Communication and Optimization (EESCO)}, pages 1--5. IEEE, 2015.

% \bibitem{c4}
% Simon Emberton, Lars Chittka, and Andrea Cavallaro.
% \newblock Underwater image and video dehazing with pure haze region segmentation.
% \newblock {\em Computer Vision and Image Understanding}, 168:145--156, 2018.

% \bibitem{c5}
% Ozan Erat, Karen Panetta, and Sos Agaian.
% \newblock Contrast enhancement for underwater images in maritime border protection.
% \newblock In {\em 2017 IEEE International Symposium on Technologies for Homeland Security (HST)}, pages 1--5. IEEE, 2017.

% \bibitem{c6}
% Fahimeh Farhadifard, Zhiliang Zhou, and Uwe Freiherr von Lukas.
% \newblock Learning-based underwater image enhancement with adaptive color mapping.
% \newblock In {\em 2015 9th International Symposium on Image and Signal Processing and Analysis (ISPA)}, pages 48--53. IEEE, 2015.

% \bibitem{c7}
% Mehdi Fatan, Mohammad Reza Daliri, and Alireza Mohammad Shahri.
% \newblock Underwater cable detection in the images using edge classification based on texture information.
% \newblock {\em Measurement}, 91:309--317, 2016.

% \bibitem{c8}
% Xueyang Fu and Xiangyong Cao.
% \newblock Underwater image enhancement with global--local networks and compressed-histogram equalization.
% \newblock {\em Signal Processing: Image Communication}, 86:115892, 2020.

% \bibitem{c9}
% Xueyang Fu, Zhiwen Fan, Mei Ling, Yue Huang, and Xinghao Ding.
% \newblock Two-step approach for single underwater image enhancement.
% \newblock In {\em 2017 International Symposium on Intelligent Signal Processing and Communication Systems (ISPACS)}, pages 789--794. IEEE, 2017.

% \bibitem{d1}
% Adrian Galdran, David Pardo, Artzai Pic{\'o}n, and Aitor Alvarez-Gila.
% \newblock Automatic red-channel underwater image restoration.
% \newblock {\em Journal of Visual Communication and Image Representation}, 26:132--145, 2015.

\bibitem{d2}
Diksha Garg, Naresh Kumar Garg, and Munish Kumar.
\newblock Underwater image enhancement using blending of CLAHE and percentile methodologies.
\newblock {\em Multimedia Tools and Applications}, 77:26545--26561, 2018.

% \bibitem{d3}
% Ahmad Shahrizan Abdul Ghani and Nor Ashidi Mat Isa.
% \newblock Underwater image quality enhancement through composition of dual-intensity images and Rayleigh-stretching.
% \newblock {\em SpringerPlus}, 3(1):1--14, 2014.

% \bibitem{d4}
% Ahmad Shahrizan Abdul Ghani and Nor Ashidi Mat Isa.
% \newblock Underwater image quality enhancement through Rayleigh-stretching and averaging image planes.
% \newblock {\em International Journal of Naval Architecture and Ocean Engineering}, 6(4):840--866, 2014.


% \bibitem{d3}
% Ahmad Shahrizan Abdul Ghani and Nor Ashidi Mat Isa.
% \newblock Underwater image quality enhancement through composition of dual-intensity images and Rayleigh-stretching.
% \newblock {\em SpringerPlus}, 3(1):1--14, 2014.

% \bibitem{d4}
% Ahmad Shahrizan Abdul Ghani and Nor Ashidi Mat Isa.
% \newblock Underwater image quality enhancement through Rayleigh-stretching and averaging image planes.
% \newblock {\em International Journal of Naval Architecture and Ocean Engineering}, 6(4):840--866, 2014.

% \bibitem{d5}
% Ahmad Shahrizan Abdul Ghani and Nor Ashidi Mat Isa.
% \newblock Enhancement of low quality underwater image through integrated global and local contrast correction.
% \newblock {\em Applied Soft Computing}, 37:332--344, 2015.

% \bibitem{d6}
% Ahmad Shahrizan Abdul Ghani and Nor Ashidi Mat Isa.
% \newblock Underwater image quality enhancement through integrated color model with Rayleigh distribution.
% \newblock {\em Applied Soft Computing}, 27:219--230, 2015.

% \bibitem{d7}
% Ahmad Shahrizan Abdul Ghani and Nor Ashidi Mat Isa.
% \newblock Automatic system for improving underwater image contrast and color through recursive adaptive histogram modification.
% \newblock {\em Computers and Electronics in Agriculture}, 141:181--195, 2017.

% \bibitem{d8}
% Evgin Goceri.
% \newblock Analysis of deep networks with residual blocks and different activation functions: classification of skin diseases.
% \newblock In {\em 2019 Ninth International Conference on Image Processing Theory, Tools and Applications (IPTA)}, pages 1--6. IEEE, 2019.

\bibitem{d9}
Evgin Goceri.
\newblock Challenges and recent solutions for image segmentation in the era of deep learning.
\newblock In {\em 2019 Ninth International Conference on Image Processing Theory, Tools and Applications (IPTA)}, pages 1--6. IEEE, 2019.

\bibitem{e1}
Evgin Goceri.
\newblock Skin disease diagnosis from photographs using deep learning.
\newblock In {\em VipIMAGE 2019: Proceedings of the VII ECCOMAS Thematic Conference on Computational Vision and Medical Image Processing, October 16--18, 2019, Porto, Portugal}, pages 239--246. Springer, 2019.

\bibitem{e2}
Manuel Gonzalez-Rivero, Oscar Beijbom, Alberto Rodriguez-Ramirez, Dominic E.~P.~Bryant, Anjani Ganase, Yeray Gonzalez-Marrero, Ana Herrera-Reveles, Emma V.~Kennedy, Catherine J.~S.~Kim, Sebastian Lopez-Marcano, et al.
\newblock Monitoring of coral reefs using artificial intelligence: A feasible and cost-effective approach.
\newblock {\em Remote Sensing}, 12(3):489, 2020.

% \bibitem{e3}
% Qingwen Guo, Lulu Xue, Ruichun Tang, and Lingrui Guo.
% \newblock Underwater image enhancement based on the dark channel prior and attenuation compensation.
% \newblock {\em Journal of Ocean University of China}, 16:757--765, 2017.

% \bibitem{e4}
% G{\"u}r Emre G{\"u}raksin, Utku K{\"o}se, and {\"O}mer Deperl{\i}o{\u{g}}lu.
% \newblock Underwater image enhancement based on contrast adjustment via differential evolution algorithm.
% \newblock In {\em 2016 International Symposium on Innovations in Intelligent Systems and Applications (INISTA)}, pages 1--5. IEEE, 2016.

% \bibitem{e5}
% Gur Emre Guraksin, Omer Deperlioglu, and Utku Kose.
% \newblock A novel underwater image enhancement approach with wavelet transform supported by differential evolution algorithm.
% \newblock {\em Nature Inspired Optimization Techniques for Image Processing Applications}, pages 255--278, 2019.

% \bibitem{e6}
% Min Han and Chao Chen.
% \newblock Enhancing underwater image by dark channel prior and color correction.
% \newblock In {\em 2016 Sixth International Conference on Information Science and Technology (ICIST)}, pages 505--510. IEEE, 2016.

% \bibitem{e7}
% Pooja Honnutagi, V.~D.~Mytri, and Y.~S.~Lalitha.
% \newblock Fusion-based underwater image enhancement by weight map techniques.
% \newblock In {\em Recent Developments in Machine Learning and Data Analytics: IC3 2018}, pages 327--339. Springer, 2019.

% \bibitem{e8}
% Minjun Hou, Risheng Liu, Xin Fan, and Zhongxuan Luo.
% \newblock Joint residual learning for underwater image enhancement.
% \newblock In {\em 2018 25th IEEE International Conference on Image Processing (ICIP)}, pages 4043--4047. IEEE, 2018.

\bibitem{e9}
Minjun Hou, Risheng Liu, Xin Fan, and Zhongxuan Luo.
\newblock Joint residual learning for underwater image enhancement.
\newblock In {\em 2018 25th IEEE International Conference on Image Processing (ICIP)}, pages 4043--4047. IEEE, 2018.

\bibitem{f1}
Kashif Iqbal, Michael Odetayo, Anne James, Rosalina Abdul Salam, and Abdullah Zawawi Hj Talib.
\newblock Enhancing the low quality images using unsupervised colour correction method.
\newblock In {\em 2010 IEEE International Conference on Systems, Man and Cybernetics}, pages 1703--1709. IEEE, 2010.

\bibitem{f2}
Md Jahidul Islam, Youya Xia, and Junaed Sattar.
\newblock Fast underwater image enhancement for improved visual perception.
\newblock {\em IEEE Robotics and Automation Letters}, 5(2):3227--3234, 2020.

\bibitem{f3}
Geir Johnsen, Martin Ludvigsen, Asgeir S{\o}rensen, and Lars Martin Sandvik Aas.
\newblock The use of underwater hyperspectral imaging deployed on remotely operated vehicles-methods and applications.
\newblock {\em IFAC-PapersOnLine}, 49(23):476--481, 2016.

% \bibitem{f4}
% Amjad Khan, Syed Saad Azhar Ali, Aamir Saeed Malik, Atif Anwer, and Fabrice Meriaudeau.
% \newblock Underwater image enhancement by wavelet based fusion.
% \newblock In {\em 2016 IEEE International Conference on Underwater System Technology: Theory and Applications (USYS)}, pages 83--88. IEEE, 2016.

% \bibitem{f5}
% Amjad Khan, Syed Saad Azhar Ali, Atif Anwer, Syed Hasan Adil, and Fabrice M{\'e}riaudeau.
% \newblock Subsea pipeline corrosion estimation by restoring and enhancing degraded underwater images.
% \newblock {\em IEEE Access}, 6:40585--40601, 2018.

% \bibitem{f6}
% G Santhan Kumar, Unnikrishnan V Painumgal, MNV Chaitanya Kumar, and KHV Rajesh.
% \newblock Autonomous underwater vehicle for vision based tracking.
% \newblock {\em Procedia Computer Science}, 133:169--180, 2018.

% \bibitem{f7}
% Munish Kumar, Manish Kumar Jindal, Rajendra Kumar Sharma, and Simpel Rani Jindal.
% \newblock Performance evaluation of classifiers for the recognition of offline handwritten Gurmukhi characters and numerals: a study.
% \newblock {\em Artificial Intelligence Review}, 53:2075--2097, 2020.

\bibitem{f8}
Chongyi Li, Jichang Guo, Chunle Guo, Runmin Cong, and Jiachang Gong.
\newblock A hybrid method for underwater image correction.
\newblock {\em Pattern Recognition Letters}, 94:62--67, 2017.

% \bibitem{f9}
% Chongyi Li, Chunle Guo, Wenqi Ren, Runmin Cong, Junhui Hou, Sam Kwong, and Dacheng Tao.
% \newblock An underwater image enhancement benchmark dataset and beyond.
% \newblock {\em IEEE Transactions on Image Processing}, 29:4376--4389, 2019.

% \bibitem{g1}
% Chongyi Li, Saeed Anwar, and Fatih Porikli.
% \newblock Underwater scene prior inspired deep underwater image and video enhancement.
% \newblock {\em Pattern Recognition}, 98:107038, 2020.

\bibitem{g2}
Dawei Li, Lihong Xu, and Huanyu Liu.
\newblock Detection of uneaten fish food pellets in underwater images for aquaculture.
\newblock {\em Aquacultural Engineering}, 78:85--94, 2017.

\bibitem{liu2014no}
Lixiong Liu, Bao Liu, Hua Huang, and Alan Conrad Bovik.
\newblock No-reference image quality assessment based on spatial and spectral entropies.
\newblock {\em Signal Processing: Image Communication}, 29(8):856--863, 2014.
\bibitem{g3}
Jianru Li and Yujie Li.
\newblock Underwater image restoration algorithm for free-ascending deep-sea tripods.
\newblock {\em Optics \& Laser Technology}, 110:129--134, 2019.

% \bibitem{g4}
% Jie Li, Katherine A.~Skinner, Ryan M.~Eustice, and Matthew Johnson-Roberson.
% \newblock WaterGAN: Unsupervised generative network to enable real-time color correction of monocular underwater images.
% \newblock {\em IEEE Robotics and Automation Letters}, 3(1):387--394, 2017.

% \bibitem{g5}
% Mading Li, Jiaying Liu, Wenhan Yang, Xiaoyan Sun, and Zongming Guo.
% \newblock Structure-revealing low-light image enhancement via robust retinex model.
% \newblock {\em IEEE Transactions on Image Processing}, 27(6):2828--2841, 2018.

% \bibitem{g6}
% Xiu Li, Zhixiong Yang, Min Shang, and Jing Hao.
% \newblock Underwater image enhancement via dark channel prior and luminance adjustment.
% \newblock In {\em OCEANS 2016-Shanghai}, pages 1--5. IEEE, 2016.

% \bibitem{g7}
% Yujie Li, Huimin Lu, Jianru Li, Xin Li, Yun Li, and Seiichi Serikawa.
% \newblock Underwater image de-scattering and classification by deep neural network.
% \newblock {\em Computers \& Electrical Engineering}, 54:68--77, 2016.

% \bibitem{g8}
% Yujie Li, Yin Zhang, Xing Xu, Li He, Seiichi Serikawa, and Hyoungseop Kim.
% \newblock Dust removal from high turbid underwater images using convolutional neural networks.
% \newblock {\em Optics \& Laser Technology}, 110:2--6, 2019.

% \bibitem{g9}
% Zhenbo Li, Guangyao Li, Bingshan Niu, and Fang Peng.
% \newblock Sea cucumber image dehazing method by fusion of retinex and dark channel.
% \newblock {\em IFAC-PapersOnLine}, 51(17):796--801, 2018.

% \bibitem{h1}
% Hui Liu and Lap-Pui Chau.
% \newblock Underwater image restoration based on contrast enhancement.
% \newblock In {\em 2016 IEEE International Conference on Digital Signal Processing (DSP)}, pages 584--588. IEEE, 2016.

% \bibitem{h2}
% Lixiong Liu, Bao Liu, Hua Huang, and Alan Conrad Bovik.
% \newblock No-reference image quality assessment based on spatial and spectral entropies.
% \newblock {\em Signal Processing: Image Communication}, 29(8):856--863, 2014.

% \bibitem{h3}
% Peng Liu, Guoyu Wang, Hao Qi, Chufeng Zhang, Haiyong Zheng, and Zhibin Yu.
% \newblock Underwater image enhancement with a deep residual framework.
% \newblock {\em IEEE Access}, 7:94614--94629, 2019.

% \bibitem{h4}
% Risheng Liu, Xin Fan, Ming Zhu, Minjun Hou, and Zhongxuan Luo.
% \newblock Real-world underwater enhancement: Challenges, benchmarks, and solutions under natural light.
% \newblock {\em IEEE Transactions on Circuits and Systems for Video Technology}, 30(12):4861--4875, 2020.

% \bibitem{h5}
% Huimin Lu, Yujie Li, Tomoki Uemura, Hyoungseop Kim, and Seiichi Serikawa.
% \newblock Low illumination underwater light field images reconstruction using deep convolutional neural networks.
% \newblock {\em Future Generation Computer Systems}, 82:142--148, 2018.

% \bibitem{h6}
% Jingyu Lu, Na Li, Shaoyong Zhang, Zhibin Yu, Haiyong Zheng, and Bing Zheng.
% \newblock Multi-scale adversarial network for underwater image restoration.
% \newblock {\em Optics \& Laser Technology}, 110:105--113, 2019.

\bibitem{h7}
Sanparith Marukatat.
\newblock Image enhancement using local intensity distribution equalization.
\newblock {\em EURASIP Journal on Image and Video Processing}, 2015(1):1--18, 2015.

% \bibitem{h8}
% Monika Mathur and Nidhi Goel.
% \newblock Enhancement of underwater images using white balancing and Rayleigh-stretching.
% \newblock In {\em 2018 5th International Conference on Signal Processing and Integrated Networks (SPIN)}, pages 924--929. IEEE, 2018.

\bibitem{10455905}
Lingxin Zhang, Youkun Chen, Jie Lan, and Yuzhen Niu.
\newblock MSSCE-GAN: Multi-Scale Structural and Color Enhanced Generative Adversarial Network for Unpaired Underwater Image Enhancement.
\newblock In {\em 2023 5th International Conference on Frontiers Technology of Information and Computer (ICFTIC)}, pages 837--841. IEEE, 2023.

\bibitem{8460552}
Cameron Fabbri, Md Jahidul Islam, and Junaed Sattar.
\newblock Enhancing Underwater Imagery Using Generative Adversarial Networks.
\newblock In {\em 2018 IEEE International Conference on Robotics and Automation (ICRA)}, pages 7159--7165. IEEE, 2018.

% \bibitem{h9}
% Pedram Mohammadi, Abbas Ebrahimi-Moghadam, and Shahram Shirani.
% \newblock Subjective and objective quality assessment of image: A survey.
% \newblock {\em arXiv preprint arXiv:1406.7799}, 2014.

% \bibitem{i1}
% Yan-Tsung Peng, Xiangyun Zhao, and Pamela C. Cosman.
% \newblock Single underwater image enhancement using depth estimation based on blurriness.
% \newblock In {\em 2015 IEEE International Conference on Image Processing (ICIP)}, pages 4952--4956. IEEE, 2015.

% \bibitem{i2}
% R. Priyadharsini, T. Sree Sharmila, and V. Rajendran.
% \newblock A wavelet transform based contrast enhancement method for underwater acoustic images.
% \newblock {\em Multidimensional Systems and Signal Processing}, 29:1845--1859, 2018.

% \bibitem{i3}
% Karen Panetta, Chen Gao, and Sos Agaian.
% \newblock Human-visual-system-inspired underwater image quality measures.
% \newblock {\em IEEE Journal of Oceanic Engineering}, 41(3):541--551, 2015.

% \bibitem{i4}
% Yan-Tsung Peng, Xiangyun Zhao, and Pamela C. Cosman.
% \newblock Single underwater image enhancement using depth estimation based on blurriness.
% \newblock In {\em 2015 IEEE International Conference on Image Processing (ICIP)}, pages 4952--4956. IEEE, 2015.

% \bibitem{i5}
% R. Priyadharsini, T. Sree Sharmila, and V. Rajendran.
% \newblock A wavelet transform based contrast enhancement method for underwater acoustic images.
% \newblock {\em Multidimensional Systems and Signal Processing}, 29:1845--1859, 2018.

% \bibitem{i6}
% Xi Qiao, Jianhua Bao, Lihua Zeng, Jian Zou, and Daoliang Li.
% \newblock An automatic active contour method for sea cucumber segmentation in natural underwater environments.
% \newblock {\em Computers and Electronics in Agriculture}, 135:134--142, 2017.

% \bibitem{i10}
% Xi Qiao, Jianhua Bao, Hang Zhang, Lihua Zeng, and Daoliang Li.
% \newblock Underwater image quality enhancement of sea cucumbers based on improved histogram equalization and wavelet transform.
% \newblock {\em Information Processing in Agriculture}, 4(3):206--213, 2017.

% \bibitem{i8}
% Chunmei Qing, Wenyou Huang, Siqi Zhu, and Xiangmin Xu.
% \newblock Underwater image enhancement with an adaptive dehazing framework.
% \newblock In {\em 2015 IEEE International Conference on Digital Signal Processing (DSP)}, pages 338--342. IEEE, 2015.

% \bibitem{i9}
% Daily Daleno de O. Rodrigues, Wagner F. de Barros, Jos{\'e} P. de Queiroz-Neto, Anderson G. Fontoura, and Jos{\'e} Reginaldo H. Carvalho.
% \newblock Enhancement of underwater images in low-to-high turbidity rivers.
% \newblock In {\em 2016 29th SIBGRAPI Conference on Graphics, Patterns and Images (SIBGRAPI)}, pages 233--240. IEEE, 2016.

% \bibitem{j1}
% Sonali Sankpal and Shraddha Deshpande.
% \newblock Underwater image enhancement by Rayleigh stretching with adaptive scale parameter and energy correction.
% \newblock In {\em Computing, Communication and Signal Processing: Proceedings of ICCASP 2018}, pages 935--947. Springer, 2019.

% \bibitem{j2}
% Sonali Sachin Sankpal and Shraddha Sunil Deshpande.
% \newblock Nonuniform illumination correction algorithm for underwater images using maximum likelihood estimation method.
% \newblock {\em Journal of Engineering}, 2016. Hindawi.

% \bibitem{j3}
% R. Sathya, M. Bharathi, and G. Dhivyasri.
% \newblock Underwater image enhancement by dark channel prior.
% \newblock In {\em 2015 2nd International Conference on Electronics and Communication Systems (ICECS)}, pages 1119--1123. IEEE, 2015.

% \bibitem{j4}
% Raimondo Schettini and Silvia Corchs.
% \newblock Underwater image processing: state of the art of restoration and image enhancement methods.
% \newblock {\em EURASIP Journal on Advances in Signal Processing}, 2010:1--14, 2010.


% \bibitem{h4}
% Risheng Liu, Xin Fan, Ming Zhu, Minjun Hou, and Zhongxuan Luo.
% \newblock Real-world underwater enhancement: Challenges, benchmarks, and solutions under natural light.
% \newblock {\em IEEE Transactions on Circuits and Systems for Video Technology}, 30(12):4861--4875, 2020.

% \bibitem{h5}
% Huimin Lu, Yujie Li, Tomoki Uemura, Hyoungseop Kim, and Seiichi Serikawa.
% \newblock Low illumination underwater light field images reconstruction using deep convolutional neural networks.
% \newblock {\em Future Generation Computer Systems}, 82:142--148, 2018.

\bibitem{h6}
Jingyu Lu, Na Li, Shaoyong Zhang, Zhibin Yu, Haiyong Zheng, and Bing Zheng.
\newblock Multi-scale adversarial network for underwater image restoration.
\newblock {\em Optics \& Laser Technology}, 110:105--113, 2019.

% \bibitem{h7}
% Sanparith Marukatat.
% \newblock Image enhancement using local intensity distribution equalization.
% \newblock {\em EURASIP Journal on Image and Video Processing}, 2015(1):1--18, 2015.

% \bibitem{h8}
% Monika Mathur and Nidhi Goel.
% \newblock Enhancement of underwater images using white balancing and Rayleigh-stretching.
% \newblock In {\em 2018 5th International Conference on Signal Processing and Integrated Networks (SPIN)}, pages 924--929. IEEE, 2018.

% \bibitem{10455905}
% Lingxin Zhang, Youkun Chen, Jie Lan, and Yuzhen Niu.
% \newblock MSSCE-GAN: Multi-Scale Structural and Color Enhanced Generative Adversarial Network for Unpaired Underwater Image Enhancement.
% \newblock In {\em 2023 5th International Conference on Frontiers Technology of Information and Computer (ICFTIC)}, pages 837--841. IEEE, 2023.

% \bibitem{8460552}
% Cameron Fabbri, Md Jahidul Islam, and Junaed Sattar.
% \newblock Enhancing Underwater Imagery Using Generative Adversarial Networks.
% \newblock In {\em 2018 IEEE International Conference on Robotics and Automation (ICRA)}, pages 7159--7165. IEEE, 2018.

% \bibitem{h9}
% Pedram Mohammadi, Abbas Ebrahimi-Moghadam, and Shahram Shirani.
% \newblock Subjective and objective quality assessment of image: A survey.
% \newblock {\em arXiv preprint arXiv:1406.7799}, 2014.

% \bibitem{i1}
% Yan-Tsung Peng, Xiangyun Zhao, and Pamela C. Cosman.
% \newblock Single underwater image enhancement using depth estimation based on blurriness.
% \newblock In {\em 2015 IEEE International Conference on Image Processing (ICIP)}, pages 4952--4956. IEEE, 2015.

% \bibitem{i2}
% R. Priyadharsini, T. Sree Sharmila, and V. Rajendran.
% \newblock A wavelet transform based contrast enhancement method for underwater acoustic images.
% \newblock {\em Multidimensional Systems and Signal Processing}, 29:1845--1859, 2018.

% \bibitem{i3}
% Karen Panetta, Chen Gao, and Sos Agaian.
% \newblock Human-visual-system-inspired underwater image quality measures.
% \newblock {\em IEEE Journal of Oceanic Engineering}, 41(3):541--551, 2015.

% \bibitem{i4}
% Yan-Tsung Peng, Xiangyun Zhao, and Pamela C. Cosman.
% \newblock Single underwater image enhancement using depth estimation based on blurriness.
% \newblock In {\em 2015 IEEE International Conference on Image Processing (ICIP)}, pages 4952--4956. IEEE, 2015.

% \bibitem{i5}
% R. Priyadharsini, T. Sree Sharmila, and V. Rajendran.
% \newblock A wavelet transform based contrast enhancement method for underwater acoustic images.
% \newblock {\em Multidimensional Systems and Signal Processing}, 29:1845--1859, 2018.

% \bibitem{i6}
% Xi Qiao, Jianhua Bao, Lihua Zeng, Jian Zou, and Daoliang Li.
% \newblock An automatic active contour method for sea cucumber segmentation in natural underwater environments.
% \newblock {\em Computers and Electronics in Agriculture}, 135:134--142, 2017.

% \bibitem{i10}
% Xi Qiao, Jianhua Bao, Hang Zhang, Lihua Zeng, and Daoliang Li.
% \newblock Underwater image quality enhancement of sea cucumbers based on improved histogram equalization and wavelet transform.
% \newblock {\em Information Processing in Agriculture}, 4(3):206--213, 2017.

% \bibitem{i8}
% Chunmei Qing, Wenyou Huang, Siqi Zhu, and Xiangmin Xu.
% \newblock Underwater image enhancement with an adaptive dehazing framework.
% \newblock In {\em 2015 IEEE International Conference on Digital Signal Processing (DSP)}, pages 338--342. IEEE, 2015.

% \bibitem{i9}
% Daily Daleno de O. Rodrigues, Wagner F. de Barros, Jos{\'e} P. de Queiroz-Neto, Anderson G. Fontoura, and Jos{\'e} Reginaldo H. Carvalho.
% \newblock Enhancement of underwater images in low-to-high turbidity rivers.
% \newblock In {\em 2016 29th SIBGRAPI Conference on Graphics, Patterns and Images (SIBGRAPI)}, pages 233--240. IEEE, 2016.

% \bibitem{j1}
% Sonali Sankpal and Shraddha Deshpande.
% \newblock Underwater image enhancement by Rayleigh stretching with adaptive scale parameter and energy correction.
% \newblock In {\em Computing, Communication and Signal Processing: Proceedings of ICCASP 2018}, pages 935--947. Springer, 2019.

% \bibitem{j2}
% Sonali Sachin Sankpal and Shraddha Sunil Deshpande.
% \newblock Nonuniform illumination correction algorithm for underwater images using maximum likelihood estimation method.
% \newblock {\em Journal of Engineering}, 2016. Hindawi.

% \bibitem{j3}
% R. Sathya, M. Bharathi, and G. Dhivyasri.
% \newblock Underwater image enhancement by dark channel prior.
% \newblock In {\em 2015 2nd International Conference on Electronics and Communication Systems (ICECS)}, pages 1119--1123. IEEE, 2015.

% \bibitem{j4}
% Raimondo Schettini and Silvia Corchs.
% \newblock Underwater image processing: state of the art of restoration and image enhancement methods.
% \newblock {\em EURASIP Journal on Advances in Signal Processing}, 2010:1--14, 2010.

% \bibitem{j5}
% Seiichi Serikawa and Huimin Lu.
% \newblock Underwater image dehazing using joint trilateral filter.
% \newblock {\em Computers \& Electrical Engineering}, 40(1):41--50, 2014.

% \bibitem{j6}
% Rajni Sethi, Indu Sreedevi, Om Prakash Verma, and Veni Jain.
% \newblock An optimal underwater image enhancement based on fuzzy gray world algorithm and bacterial foraging algorithm.
% \newblock In {\em 2015 Fifth National Conference on Computer Vision, Pattern Recognition, Image Processing and Graphics (NCVPRIPG)}, pages 1--4. IEEE, 2015.

% \bibitem{j7}
% Norsila bt Shamsuddin, Baharum b Baharudin, Mohd Kushairi, Mohd Rajuddin, and Farahwahida bt Mohd, et al.
% \newblock Significance level of image enhancement techniques for underwater images.
% \newblock In {\em 2012 International Conference on Computer \& Information Science (ICCIS)}, volume 1, pages 490--494. IEEE, 2012.

% \bibitem{j8}
% Supriya S. Shigwan and Gajanan K. Birajdar.
% \newblock Objective image quality assessment using perceptual distortion for image retargeting.
% \newblock In {\em 2015 1st International Conference on Next Generation Computing Technologies (NGCT)}, pages 955--959. IEEE, 2015.

% \bibitem{j9}
% Snehan Shourya, Sumit Kumar, and Rajib Kumar Jha.
% \newblock Adaptive fractional differential approach to enhance underwater images.
% \newblock In {\em 2016 Sixth International Symposium on Embedded Computing and System Design (ISED)}, pages 56--60. IEEE, 2016.

% \bibitem{k1}
% Gajraj Singh, Neena Jaggi, Srikanth Vasamsetti, H. K. Sardana, Satish Kumar, and Neerja Mittal.
% \newblock Underwater image/video enhancement using wavelet based color correction (WBCC) method.
% \newblock In {\em 2015 IEEE Underwater Technology (UT)}, pages 1--5. IEEE, 2015.

% \bibitem{k2}
% Ritu Singh and Mantosh Biswas.
% \newblock Adaptive histogram equalization based fusion technique for hazy underwater image enhancement.
% \newblock In {\em 2016 IEEE International Conference on Computational Intelligence and Computing Research (ICCIC)}, pages 1--5. IEEE, 2016.

% \bibitem{k3}
% Ritu Singh and Mantosh Biswas.
% \newblock Contrast and color improvement based haze removal of underwater images using fusion technique.
% \newblock In {\em 2017 4th International Conference on Signal Processing, Computing and Control (ISPCC)}, pages 138--143. IEEE, 2017.

% \bibitem{k4}
% K. Srividhya and M. M. Ramya.
% \newblock Performance analysis of pre-processing filters for underwater images.
% \newblock In {\em 2015 International Conference on Robotics, Automation, Control and Embedded Systems (RACE)}, pages 1--7. IEEE, 2015.

% \bibitem{k5}
% Xin Sun, Lipeng Liu, and Junyu Dong.
% \newblock Underwater image enhancement with encoding-decoding deep CNN networks.
% \newblock In {\em 2017 IEEE SmartWorld, Ubiquitous Intelligence \& Computing, Advanced \& Trusted Computed, Scalable Computing \& Communications, Cloud \& Big Data Computing, Internet of People and Smart City Innovation (SmartWorld/SCALCOM/UIC/ATC/CBDCom/IOP/SCI)}, pages 1--6. IEEE, 2017.





%%% Uncomment this section and comment out the \bibliography{references} line above to use inline references.
% \begin{thebibliography}{1}

% 	\bibitem{kour2014real}
% 	George Kour and Raid Saabne.
% 	\newblock Real-time segmentation of on-line handwritten arabic script.
% 	\newblock In {\em Frontiers in Handwriting Recognition (ICFHR), 2014 14th
% 			International Conference on}, pages 417--422. IEEE, 2014.

% 	\bibitem{kour2014fast}
% 	George Kour and Raid Saabne.
% 	\newblock Fast classification of handwritten on-line arabic characters.
% 	\newblock In {\em Soft Computing and Pattern Recognition (SoCPaR), 2014 6th
% 			International Conference of}, pages 312--318. IEEE, 2014.

% 	\bibitem{hadash2018estimate}
% 	Guy Hadash, Einat Kermany, Boaz Carmeli, Ofer Lavi, George Kour, and Alon
% 	Jacovi.
% 	\newblock Estimate and replace: A novel approach to integrating deep neural
% 	networks with existing applications.
% 	\newblock {\em arXiv preprint arXiv:1804.09028}, 2018.





